Dynamic Geometric Set Cover, Revisited

Geometric set cover is a classical problem in computational geometry, which has been extensively studied in the past. In the dynamic version of the problem, points and ranges may be inserted and deleted, and our goal is to efficiently maintain a set cover solution (satisfying certain quality requirement). In this paper, we give a plethora of new dynamic geometric set cover data structures in 1D and 2D, which significantly improve and extend the previous results: 1. The first data structure for $(1+\varepsilon)$-approximate dynamic interval set cover with polylogarithmic amortized update time. Specifically, we achieve an update time of $O(\log^3 n/\varepsilon)$, improving the $O(n^\delta/\varepsilon)$ bound of Agarwal et al. [SoCG'20], where $\delta>0$ denotes an arbitrarily small constant. 2. A data structure for $O(1)$-approximate dynamic unit-square set cover with $2^{O(\sqrt{\log n})}$ amortized update time, substantially improving the $O(n^{1/2+\delta})$ update time of Agarwal et al. [SoCG'20]. 3. A data structure for $O(1)$-approximate dynamic square set cover with $O(n^{1/2+\delta})$ randomized amortized update time, improving the $O(n^{2/3+\delta})$ update time of Chan and He [SoCG'21]. 4. A data structure for $O(1)$-approximate dynamic 2D halfplane set cover with $O(n^{17/23+\delta})$ randomized amortized update time. The previous solution for halfplane set cover by Chan and He [SoCG'21] is slower and can only report the size of the approximate solution. 5. The first sublinear results for the \textit{weighted} version of dynamic geometric set cover. Specifically, we give a data structure for $(3+o(1))$-approximate dynamic weighted interval set cover with $2^{O(\sqrt{\log n \log\log n})}$ amortized update time and a data structure for $O(1)$-approximate dynamic weighted unit-square set cover with $O(n^\delta)$ amortized update time.

==> overview.tex <==
\section{Unweighted Interval Set Cover} \label{sec-shortint}
Let $(S,\mathcal{I})$ be a dynamic unweighted interval set cover instance where $S$ is the set of points and $\mathcal{I}$ is the set of intervals, and let $\varepsilon >0$. % be the approximation factor.
We show how to design a data structure $\mathcal{D}$ that maintains a $(1+\varepsilon)$-approximate set cover solution for $(S,\mathcal{I})$.
W.l.o.g., we assume that the points in $S$ are always in the range $[0,1]$, which we call the \textit{point range} of $(S,\mathcal{I})$.

Let $r$ and $\alpha < 1$ be two parameters to be determined.
To design $\mathcal{D}$, our basic idea is to partition the instance $(S,\mathcal{I})$ into smaller ``sub-instances'', recursively build data structures to maintain solutions for the sub-instances, and obtain the set cover for $(S,\mathcal{I})$ by properly combining the solutions of the sub-instances.
Specifically, we partition the point range $[0,1]$ into $r$ portions $J_1,\dots,J_r$ such that each $J_i$ contains $O(n/r)$ points in $S$ and $O(n/r)$ endpoints of intervals in $\mathcal{I}$.
We define $S_i = S \cap J_i$ and $\mathcal{I}_i = \{I \in \mathcal{I}: I \cap J_i \neq \emptyset \text{ and } J_i \nsubseteq I\}$.
When $(S,\mathcal{I})$ changes, the portions $J_1,\dots,J_r$ remain unchanged while the $S_i$'s and $\mathcal{I}_i$'s will change along with $S$ and $\mathcal{I}$.
We view each $(S_i,\mathcal{I}_i)$ as a dynamic interval set cover instance with point range $J_i$ (called a \textit{sub-instance}) and recursively build a dynamic interval set cover data structure $\mathcal{D}_i$ (called a \textit{sub-structure}) which maintains a $(1+\tilde{\varepsilon})$-approximate set cover solution for $(S_i,\mathcal{I}_i)$ with $\tilde{\varepsilon} = \alpha \varepsilon$.
We reconstruct the entire data structure after $n/r$ operations (this guarantees the size of each sub-instance $(S_i,\mathcal{I}_i)$ is always $O(n/r)$).

%\vspace{-0.3cm}

\subsubsection*{Constructing a solution.}
Given the set cover solutions of the sub-instances, we can obtain a set cover of $(S,\mathcal{I})$ as follows.
For each $i \in [r]$, if $J_i$ can be covered by an interval $I \in \mathcal{I}$, we define $\mathcal{I}_i^* = \{I\}$, otherwise let $\mathcal{I}_i^*$ be the $(1+\tilde{\varepsilon})$-approximate solution for $(S_i,\mathcal{I}_i)$ maintained in $\mathcal{D}_i$.
Then we define $\mathcal{I}_\text{appx} = \bigsqcup_{i=1}^r \mathcal{I}_i^*$.
% , which is clearly a set cover of $(S,\mathcal{I})$.
We observe that $\mathcal{I}_\text{appx}$ is a $(1+\tilde{\varepsilon})$-approximate solution of $(S,\mathcal{I})$ with an $O(r)$ additive error.
%Let $\mathsf{opt}$ denote the size of an optimal set cover of $(S,\mathcal{I})$.
\begin{fact} \label{fact-intquality}
$|\mathcal{I}_\textnormal{appx}| \leq (1+\tilde{\varepsilon}) \cdot \mathsf{opt} + O(r)$.
%where $\mathsf{opt}$ is the size of an optimal set cover of $(S,\mathcal{I})$.
\end{fact}
By this observation, if $\mathsf{opt}$ is large, namely, $\mathsf{opt} \geq c \cdot r/(\varepsilon-\tilde{\varepsilon}) = c \cdot r / (\varepsilon - \alpha \varepsilon)$ for a sufficiently large constant $c$, then $|\mathcal{I}_\text{appx}| \leq (1+\varepsilon) \cdot \mathsf{opt}$.
%In this case, we already solve the problem.
On the other hand, if $\mathsf{opt}$ is small, then
an optimal solution of $(S,\mathcal{I})$ can be computed easily in \textit{output-sensitive} time by the following lemma.

\begin{lemma} \label{lem-intos}
One can store a dynamic (unweighted) interval set cover instance $(S,\mathcal{I})$ in a data structure $\mathcal{A}$ with $O(n\log n)$ construction time and $O(\log n)$ update time such that at any point, an optimal solution for $(S,\mathcal{I})$ can be computed in $O(\mathsf{opt} \cdot \log n)$ time with the access to $\mathcal{A}$.
\end{lemma}
%When $\mathsf{opt} < c \cdot r \log n/\varepsilon$, we can apply the algorithm of Lemma~\ref{lem-intos} to compute an optimal set cover of $(S,\mathcal{I})$ in $\widetilde{O}(\mathsf{opt}) = \widetilde{O}(r/\varepsilon)$ time.
\noindent
%Therefore, our strategy is the following.
We first simulate the algorithm of Lemma~\ref{lem-intos} within $\widetilde{O}(r/(\varepsilon - \alpha \varepsilon))$ time.
If the algorithm outputs an optimal set cover of $(S,\mathcal{I})$, we are done.
Otherwise, $\mathsf{opt} \geq c \cdot r \log n/\varepsilon$ and hence $\mathcal{I}_\text{appx}$ defined above is a $(1+\varepsilon)$-approximate solution of $(S,\mathcal{I})$.

Now we briefly discuss how to answer the queries to the solution efficiently.
If the solution is computed by the algorithm of Lemma~\ref{lem-intos}, then we have all the intervals used in the solution and we can store them in a data structure (such as a binary search tree) which supports the desired queries.
If the solution is defined as $\mathcal{I}_\text{appx} = \bigsqcup_{i=1}^r \mathcal{I}_i^*$, its size might be large and thus we cannot extract all the intervals in the solution.
Fortunately, the set cover solutions of the sub-instances are already maintained in the sub-structures (which supports the queries).
Thus, we only need to store those $\mathcal{I}_i^*$'s which consist of a single interval covering $J_i$.

%\vspace{-0.3cm}

\subsubsection*{Analysis.}
The update time of our data structures basically consist of three parts: the time for recursively updating the sub-structures, the time for constructing the solution, and the time for reconstruction.
It is easy to see that the last two parts can be done in $\widetilde{O}(r/(\varepsilon - \alpha \varepsilon))$ (amortized) time.
To consider the time for recursive updates, we notice the depth of the recursion is $O(\log_r n)$.
If we set $\alpha = 1-1/\log_r n$, the approximation parameter in any level of the recursion is $\Theta(\varepsilon)$.
%\TIMOTHY{technically, $1+\Theta(\eps)$... or should that be $1+\tilde{\eps}$?  (and inconsistency with previous page, where we are precise about approximation factor without big-O?)}
%\Jie{What I meant is that in every level of the recursion, the approximation parameter ``eps'' is $\Theta(\eps)$. It will become smaller and smaller but still lower bounded by $\Omega(\varepsilon)$. Therefore, when we analyze the update time we do not need to include $\eps$ in the recurrence.}
For point insertion/deletion, we only need to recursively update one sub-structure because only one sub-instance changes.
So if we use $U(n)$ to denote the update time when the instance size is $n$, we have the recurrence $U(n) = U(O(n/r)) + \widetilde{O}(r/(\varepsilon - \alpha \varepsilon))$ for point insertions/deletions, which solves to $U(n) = \widetilde{O}(r \log_r n /(\varepsilon - \alpha \varepsilon))) = \widetilde{O}(r \log_r^2 n/\varepsilon)$.
For interval insertion/deletion, we distinguish two cases.
We say an interval in $\mathcal{I}$ is \textit{two-sided} if both of its endpoints are in the point range $[0,1]$, and \textit{one-sided} otherwise.
An insertion/deletion of a one-sided interval only changes one sub-instance, and hence the update time satisfies the same recurrence above and is $\widetilde{O}(r \log_r^2 n/\varepsilon)$.
An insertion/deletion of a two-sided interval can change one or two sub-instances.
The key observation here is that, if two sub-instances $(S_i,\mathcal{I}_i)$ and $(S_j,\mathcal{I}_j)$ are changed, then the two endpoints of the inserted/deleted interval belong to $J_i$ and $J_j$ respectively.
Thus, the inserted/deleted interval is a \textit{one-sided} interval in $(S_i,\mathcal{I}_i)$ and $(S_j,\mathcal{I}_j)$.
In other words, the recursive updates on $\mathcal{D}_i$ and $\mathcal{D}_j$ are one-sided interval updates, which takes $\widetilde{O}(r \log_r^2 n /\varepsilon)$ time.
So the update time for two-sided intervals satisfies
\begin{equation*}
    U_1(n) = \max\{U_1(O(n/r)), \widetilde{O}(r \log_r^2 n/\varepsilon)\} + \widetilde{O}(r/(\varepsilon - \alpha \varepsilon)),
\end{equation*}
which again solves to $U_1(n) = \widetilde{O}(r \log_r^2 n/\varepsilon)$.
By setting $r$ to be a sufficiently large constant, the (amortized) update time of our data structure is then $\widetilde{O}(1 /\varepsilon)$ (more precisely, $O(\log^3 n/\varepsilon)$).
We omit the details and the analysis for the query times, which can be found in the full paper.
%Section~\ref{sec-unweightedint}.

\begin{restatable}{theorem}{unweightedint} \label{thm-unweightedint}
There exists a dynamic data structure for $(1+\varepsilon)$-approximate unweighted interval set cover with $O(\log^3 n/\varepsilon)$ amortized update time and $\widetilde{O}(n)$ construction time, which can answer size, membership, and reporting queries in $O(1)$, $O(\log n)$, and $O(k \log n)$ time, respectively, where $n$ is the size of the instance and $k$ is the size of the maintained solution.
\end{restatable}

%\vspace{-0.3cm}

\ignore{
\subsubsection*{Remark.}
The basic idea of partitioning into sub-instance, using the output-sensitive algorithm when $\mathsf{opt}$ is small and otherwise combining the solutions of the sub-instances is somewhat routine,  and it also underlies the previous work~\cite{agarwal2020dynamic}.
To improve on the $O(n^\delta)$ update bound, however, requires a careful application of this approach, combined with two simple but crucial ideas:
introducing the notion of point ranges and distinguishing one-sided intervals from two-sided ones in the analysis.
While these ideas are technically simple, they turn out to be key to improving the update time from polynomial to poly-logarithmic.
}
%We notice that besides the recursive update

%We consider two cases: $\mathsf{opt}$ is small and $\mathsf{opt}$ is large.
%Set $\delta = c \cdot r \log n /\varepsilon$ as a threshold where $c$ is a sufficiently large constant.
%If $\mathsf{opt} \leq \delta$, then we can use the output-sensitive algorithm of Lemma~\ref{lem-intos} to compute an optimal set cover of $(S,\mathcal{I})$ in $\widetilde{O}(\mathsf{opt}) = \widetilde{O}(\delta) = \widetilde{O}(r/\varepsilon)$ time.

\section{Unweighted Unit-Square Set Cover}\label{unweighted unit-square}
The dynamic set cover of unit-squares can be maintained with the same update time as set cover of \emph{quadrants} at the loss of only a constant factor in the approximation ratio, as observed in Agarwal et al.'s paper~\cite{agarwal2020dynamic}. The quadrant problem also admits a (constant factor) \textit{output-sensitive} algorithm.

\begin{lemma}[\cite{agarwal2020dynamic}] \label{lem-quados}
One can store a dynamic (unweighted) quadrant set cover instance $(S,\mathcal{Q})$ in a data structure $\mathcal{A}$ with $\widetilde{O}(n)$ construction time and $\widetilde{O}(1)$ update time such that at any point, a constant-approximate solution for $(S,\mathcal{Q})$ can be computed in $\widetilde{O}(\mathsf{opt})$ time with the access to $\mathcal{A}$.
\end{lemma}
Let $(S,\mathcal{Q})$ be a dynamic (unweighted) quadrant set cover instance where $S$ is the set of points in $\mathbb{R}^2$ and $\mathcal{Q}$ is the set of quadrants.
Suppose $\mu = O(1)$ is the approximation factor of the algorithm of Lemma~\ref{lem-quados}.
We show how to design a data structure $\mathcal{D}$ that maintains a $(\mu+\varepsilon)$-approximate solution for $(S,\mathcal{Q})$ for a given $\varepsilon>0$.
W.l.o.g., we assume that the points in $S$ are always in the \textit{point range} $[0,1]^2$.
We say a quadrant in $\mathcal{Q}$ is \textit{trivial} (resp., \textit{nontrivial}) if its vertex is outside (resp., inside) the point range $[0,1]^2$.

The basic idea again is to partition $(S,\mathcal{Q})$ into smaller sub-instances, recursively build sub-structures for these sub-instances, and properly combine the solutions of the sub-instances to obtain a solution for $(S,\mathcal{Q})$.
Specifically, we partition the point range $[0,1]^2$ into $r \times r$ rectangular cells using $r-1$ horizontal/vertical lines such that each row (resp., column) of $r$ cells contains $O(n/r)$ points in $S$ and $O(n/r)$ vertices of quadrants in $\mathcal{Q}$.
Let $\Box_{i,j}$ be the cell in the $i$-th row and $j$-th column for $(i,j) \in [r]^2$.
%Also, let $R_i = \bigcup_{j=1}^r \Box_{i,j}$ and $C_j = \bigcup_{i=1}^r \Box_{i,j}$, i.e., $R_i$ is the $i$-th row of the partition and $C_j$ the $j$-th column of the partition.
Define $S_{i,j} = S \cap \Box_{i,j}$ for $i,j \in [r]$.
Next, we define $\mathcal{Q}_{i,j} \subseteq \mathcal{Q}$ for $i,j \in [r]$ as follows.
We include in $\mathcal{Q}_{i,j}$ all \textit{nontrivial} quadrants whose vertices lie in $\Box_{i,j}$.
Then we consider the nontrivial quadrants partially intersecting $\Box_{i,j}$ (i.e., intersecting but not containing $\Box_{i,j}$) whose vertices are not in $\Box_{i,j}$.
These quadrants must contain one of the left, right, top, bottom boundaries of $\Box_{i,j}$.
Thus, among these quadrants, there are (at most) four quadrants which have maximal intersections with $\Box_{i,j}$.
We include in $\mathcal{Q}_{i,j}$ these four quadrants.
Note that all quadrants in $\mathcal{Q}_{i,j}$ are nontrivial.
We view each $(S_{i,j},\mathcal{Q}_{i,j})$ as a dynamic quadrant instance and recursively build a data structure $\mathcal{D}_{i,j}$ which maintains a $(\mu+\tilde{\varepsilon})$-approximate set cover solution for $(S_i,\mathcal{I}_i)$ with $\tilde{\varepsilon} = \alpha \varepsilon$.
Besides the cells, we also define sub-instances for the rows/columns of the partition.
Specifically, let $R_i = \bigcup_{j=1}^r \Box_{i,j}$ and $C_j = \bigcup_{i=1}^r \Box_{i,j}$, i.e., $R_i$ is the $i$-th row of the partition and $C_j$ the $j$-th column of the partition.
Define $S_{i,\bullet} = S \cap R_i$ and $S_{\bullet,j} = S \cap C_j$, for $i,j \in [r]$.
Then we define the quadrant sets $\mathcal{Q}_{i,\bullet}$ and $\mathcal{Q}_{\bullet,j}$ in the same way as above: $\mathcal{Q}_{i,\bullet}$ (resp., $\mathcal{Q}_{\bullet,j}$) consists of all nontrivial quadrants whose vertices are in $R_i$ (resp., $C_j$) and up to four maximal nontrivial quadrants which partially intersect $R_i$ (resp., $C_j$) and have vertices are not in $R_i$ (resp., $C_j$).
Also, we recursively build a data structure $\mathcal{D}_{i,\bullet}$ (resp., $\mathcal{D}_{\bullet,j}$) that maintains a $(\mu+\tilde{\varepsilon})$-approximate set cover solution for $(S_{i,\bullet},\mathcal{Q}_{i,\bullet})$ (resp., $(S_{\bullet,j},\mathcal{Q}_{\bullet,j})$).
We reconstruct the entire data structure after $n/r$ operations.

%\vspace{-0.3cm}

\subsubsection*{Constructing a solution.}
Let $\mathsf{opt}$ be the size of an optimal set cover of $(S,\mathcal{Q})$.
The high-level idea to construct a $(\mu+\varepsilon)$-approximate set cover solution for $(S,\mathcal{Q})$ is similar to what we used in dynamic interval set cover.
If $\mathsf{opt}$ is small, we can run the output-sensitive algorithm of Lemma~\ref{lem-quados} to compute a $\mu$-approximate solution.
%otherwise we construct the solution for $(S,\mathcal{Q})$ by properly combining the solutions maintained in the sub-structures.
Otherwise, we construct a solution $\mathcal{Q}_\text{appx}$ for $(S,\mathcal{Q})$ with certain \textit{additive} error by properly combining the solutions maintained in the sub-structures, which turns out to be a $(\mu+\varepsilon)$-approximate solution because $\mathsf{opt}$ is large in this case.
The difficulty here is clearly how to combine the solutions maintained in the sub-structures to obtain the desired set cover $\mathcal{Q}_\text{appx}$.
To this end, we first consider the trivial quadrants in $\mathcal{Q}$.
There are (at most) four trivial quadrants which have maximal intersections with $[0,1]^2$; they contain the top, bottom, left, right boundaries of $[0,1]^2$, respectively (we denote by $Q_\uparrow,Q_\downarrow,Q_\leftarrow,Q_\rightarrow$).
All other trivial quadrants are useless because their coverage is dominated by one of these four.
Furthermore, we can always include $Q_\uparrow,Q_\downarrow,Q_\leftarrow,Q_\rightarrow$ in $\mathcal{Q}_\text{appx}$ because doing this can only increase the additive error by 4.
Then the remaining task is to use the nontrivial quadrants in $\mathcal{Q}$ to cover the points in $S$ that are not covered by $Q_\uparrow,Q_\downarrow,Q_\leftarrow,Q_\rightarrow$.
The complement of the union of $Q_\uparrow,Q_\downarrow,Q_\leftarrow,Q_\rightarrow$ in $[0,1]^2$ is a rectangle, which we denote by $X$.
For each cell $\Box_{i,j} \subseteq X$, if there exists a quadrant $Q \in \mathcal{Q}$ that contains $\Box_{i,j}$, we define $\mathcal{Q}_{i,j}^* = \{Q\}$, otherwise let $\mathcal{Q}_{i,j}^*$ be the set cover of $(S_{i,j},\mathcal{Q}_{i,j})$ maintained in the sub-structure $\mathcal{D}_{i,j}$.
We then add the quadrants in these $\mathcal{Q}_{i,j}^*$'s to $\mathcal{Q}_\text{appx}$.
By doing this, all points in $S$ are covered except those in a rectangular annulus which is the complement of the union of the cells $\Box_{i,j} \subseteq X$ in $X$ (see Figure~\ref{fig-annulus}).
We partition this rectangular annulus into four rectangles $L_\uparrow,L_\downarrow,L_\leftarrow,L_\rightarrow$ (again see Figure~\ref{fig-annulus}), each of which is contained in a row $R_i$ or a column $C_j$.
We obtain a set cover for the points in each of $L_\uparrow,L_\downarrow,L_\leftarrow,L_\rightarrow$ using the corresponding row/column sub-structure as follows.
Consider $L_\uparrow$ and suppose $L_\uparrow \subseteq R_i$.
We temporarily insert the three quadrants $Q_\uparrow,Q_\leftarrow,Q_\rightarrow$ to $\mathcal{Q}_{i,\bullet}$ (these quadrants will be deleted afterwards) and update the sub-structure $\mathcal{D}_{i,\bullet}$ so that $\mathcal{D}_{i,\bullet}$ now maintains a solution for $(S_{i,\bullet},\mathcal{Q}_{i,\bullet} \cup \{Q_\uparrow,Q_\leftarrow,Q_\rightarrow\})$.
This solution covers all points in $S \cap L_\uparrow$ (as it covers $S_{i,\bullet}$) and one can verify that it is a $(\mu+\tilde{\varepsilon})$-approximate set cover solution for $(S \cap L_\uparrow, \mathcal{Q})$ with a constant additive error.
In this way, we can obtain set covers for the points in $L_\uparrow,L_\downarrow,L_\leftarrow,L_\rightarrow$ and then include these quadrants to our solution $\mathcal{Q}_\text{appx}$.
Similar to Fact~\ref{fact-intquality}, we can show that $\mathcal{Q}_\textnormal{appx}$ is a $(\mu+\tilde{\varepsilon})$-approximate solution for $(S,\mathcal{Q})$ with an $O(r^2)$ additive error.
\begin{fact}
$|\mathcal{Q}_\textnormal{appx}| \leq (\mu+\tilde{\varepsilon}) \cdot \mathsf{opt} + O(r^2)$, where $\mathsf{opt}$ is the size of an optimal set cover of $(S,\mathcal{Q})$.
\end{fact}

\begin{figure}[t]
    \centering
    \includegraphics[height=2.8cm]{annulus.pdf}
    \caption{The rectangular annulus (the grey area) are partitioned into four rectangles.}
    \label{fig-annulus}
\end{figure}

If $\mathsf{opt} \geq c \cdot r^2 /(\varepsilon - \alpha \varepsilon)$, then $\mathcal{Q}_\textnormal{appx}$ is a $(\mu+\varepsilon)$-approximate solution for $(S,\mathcal{Q})$.
In the case $\mathsf{opt} < c \cdot r^2 /(\varepsilon - \alpha \varepsilon)$, we can use the output-sensitive algorithm of Lemma~\ref{lem-quados} to compute a $\mu$-approximate solution for $(S,\mathcal{Q})$ in $\widetilde{O}(r^2/(\varepsilon - \alpha \varepsilon))$ time.
The way to store the solution for answering queries is similar to that in dynamic interval set cover (but slightly more complicated), and we omit the details here.

%\vspace{-0.3cm}

\subsubsection*{Analysis.}
Here we only analyze the update time for quadrant insertions/deletions (the analysis for point insertions/deletions is simpler).
Excluding the time cost for recursively updating the sub-structures, each update of our data structure takes $\widetilde{O}(r^2/(\varepsilon - \alpha \varepsilon) + r^2 \cdot 2^{O(\log_r n)})$ (amortized) time.
To see the time cost for recursive updates, we notice the depth of the recursion is $O(\log_r n)$.
If we set $\alpha = 1- 1/\log_r n$, the approximation factor in any level of the recursion is $\Theta(\varepsilon)$.
Now we distinguish two cases according to whether the inserted/deleted quadrant $Q$ is trivial.
If $Q$ is trivial, the sub-instances do not change because the sets $\mathcal{Q}_{i,j},\mathcal{Q}_{i,\bullet},\mathcal{Q}_{\bullet,j}$ only contain nontrivial quadrants.
But we still need a constant number of recursive updates when we construct the set covers for the points in $L_\uparrow,L_\downarrow,L_\leftarrow,L_\rightarrow$ (we need to temporarily insert some quadrants to the row/column sub-instances and delete them afterwards).
Note that all of these updates are \textit{trivial} quadrant updates.
If $Q$ is nontrivial, let $i,j \in [r]$ such that the vertex of $Q$ is contained in $\Box_{i,j}$.
Then we need to recursively update $O(r)$ sub-structures, in which only the updates for $\mathcal{D}_{i,j},\mathcal{D}_{i,\bullet},\mathcal{D}_{\bullet,j}$ are nontrivial quadrant updates (because the vertex of $Q$ is outside the point ranges of all the other sub-instances).
To summarize, a trivial quadrant update requires $O(1)$ recursive trivial updates and a nontrivial quadrant update requires $O(1)$ recursive nontrivial updates and $O(r)$ recursive trivial updates.
Hence, if we use $U_1(n)$ and $U_2(n)$ to denote the update time for trivial and nontrivial quadrant updates, then we have the recurrences
\begin{equation*}
    U_1(n) = O(1) \cdot U_1(O(n/r)) + \widetilde{O}(r^2/(\varepsilon - \alpha \varepsilon) + r^2 \cdot 2^{O(\log_r n)}),
\end{equation*}
\begin{equation*}
    U_2(n) = O(1) \cdot U_2(O(n/r)) + O(r) \cdot U_1(O(n/r)) + \widetilde{O}(r^2/(\varepsilon - \alpha \varepsilon) + r^2 \cdot 2^{O(\log_r n)}).
\end{equation*}
The first recurrence solves to $U_1(n) = \widetilde{O}((r^2/\varepsilon) \cdot 2^{O(\log_r n)})$.
With this in hand, we can solve the second recurrence to obtain $U_2(n) = \widetilde{O}((r^3/\varepsilon) \cdot 2^{O(\log_r n)})$.
%If $Q$ is nontrivial, let $i,j \in [r]$ such that the vertex of $Q$ is contained in $\Box_{i,j}$.
%Then we need to recursively update $O(r)$ sub-structures, in which only the updates for $\mathcal{D}_{i,j},\mathcal{D}_{i,\bullet},\mathcal{D}_{\bullet,j}$ are nontrivial quadrant updates (because the vertex of $Q$ is outside the point ranges of all the other sub-instances).
%Thus, in this case, we need $O(1)$ recursive nontrivial quadrant updates and $O(r)$ trivial ones, and the update time satisfies
%\begin{equation*}
%    U(n) = O(1) \cdot U(O(n/r)) + \widetilde{O}((r^2/\varepsilon) \cdot 2^{O(\log_r n)}),
%\end{equation*}
%which also solves to $U(n) = \widetilde{O}((r^2/\varepsilon) \cdot 2^{O(\log_r n)})$.
Setting $r = 2^{\sqrt{\log n}}$ and $\varepsilon$ be any constant, we achieve $2^{O(\sqrt{\log n})}$ update time with $O(1)$ approximation ratio.

\begin{restatable}{theorem}{unweightedusq} \label{thm-unweightedusq}
There exists a dynamic data structure for $O(1)$-approximate unweighted unit-square set cover with $2^{O(\sqrt{\log n})}$ amortized update time and $2^{O(\sqrt{\log n})} \cdot n$ construction time, which can answer size, membership, and reporting queries in $O(1)$, $2^{O(\sqrt{\log n})}$, and $O(k \sqrt{\log n})$ time, respectively, where $n$ is the size of the instance and $k$ is the size of the maintained solution.
\end{restatable}

%If a quadrant $Q \in \mathcal{Q}$ partially intersects $\Box_{i,j}$ (i.e., $Q \cap \Box_{i,j} \neq \emptyset$ and $\Box_{i,j} \nsubseteq Q$) and the vertex of $Q$ does not lie in $\Box$, then $Q$ must contains one of the top, bottom, left, right boundaries of $\Box_{i,j}$.
%There are (at most) four such quadrants in $\mathcal{Q}$ which have maximal intersections with $\Box_{i,j}$; .

\section{Unweighted Square Set Cover}
\ignore{
In this section, we briefly explain our ideas for $O(1)$-approximate dynamic square set cover. Our data structure is based on the previous method by \cite{chan2021dynamic} (with $O(n^{2/3+\delta})$ update time), which recursively partitions the space using a quadtree, until getting $\tilde{O}(\frac{n}{b})$ leaf cells each with size $O(b)$ for a parameter $b$. They then decompose each leaf cell into canonical rectangles with total size $b^{1+O(\delta)}$, such that any query rectangle in the cell can be decomposed into $O(1)$ canonical rectangles. The global solution is obtained by taking the union of a subset of the canonical rectangles in the leaf cells.

In our new approach, instead of maintaining an approximate solution in each canonical rectangle using the static set cover algorithm, we classify the canonical rectangles into \emph{heavy} and \emph{light}. The intuition is that to balance the query and update time, we build a subquadtree for each of the heavy ones to maintain the approximate solution during updates, but compute the solutions from scratch for the light ones during queries. By a more careful choice of parameters, we are able to balance the query and update time to $O(n^{1/2+\delta})$. The details are deferred to the full paper.
}
%Let $(S,\mathcal{I})$ be a dynamic (unweighted) square set cover instance where $S$ is the set of points in $\mathbb{R}$ and $\mathcal{I}$ is the set of squares. Let $n=|S|+|\mathcal{I}|$ denote the instance size.

In the 2D unweighted square case,
we obtain the following result, by
modifying Chan and He's previous
data structure~\cite{ChanH20}.  The details
are given in the full paper.

\begin{theorem}
There exists a dynamic data structure for $O(1)$-approximate unweighted square set cover with $O(n^{1/2+\delta})$ query and update time with high probability (w.h.p.), for any constant $\delta>0$.
%and $O(n^{1+\delta})$ construction time
\end{theorem}

%\TIMOTHY{These two paragraphs may not be very meaningful to people who don't know the previous paper (and the intro already said the same thing) -- maybe just delete, and say this case is deferred to full paper?}
%\Qizheng{Ok, makes sense. Do we still need to keep the section heading and the theorem statement?}


\section{Unweighted 2D Halfplane Set Cover}
In this section, we present a data structure for $O(1)$-approximate dynamic 2D halfplane set cover. Previously, Chan and He \cite{chan2021dynamic} provided a dynamic set cover structure for 3D halfspace with $O(n^{12/13+\delta})$ update time, which clearly also holds for 2D halfplanes, but their scheme is unable to actually find a set cover---it only reports its size. We not only improve the update time, but can also find the approximate set cover solution.

Let $(S,\mathcal{H})$ be a dynamic (unweighted) 2D halfplanes set cover instance where $S$ is a set of points in $\mathbb{R}^2$ and $\mathcal{H}$ is a set of halfplanes, with $m=|S|$ and $n=|\mathcal{H}|$. We use $N = n+m$ to denote the global instance size. Here we present a solution that only supports halfplane insertion/deletions and point deletions; the ways to support point insertions are more technical, and the details are deferred to the full version.

\subsubsection*{Algorithm for small opt.} We first note that there is an algorithm that is efficient when $\mathsf{opt}$ is small, which will be used later as a subroutine. The idea is to modify the small $\mathsf{opt}$ algorithm for axis-aligned squares by Chan and He \cite{chan2021dynamic}, which is based on an efficient implementation of the randomized multiplicative weight update method. In this way, we obtain update time $\widetilde{O}(z)$ and query time $\widetilde{O}(\mathsf{opt}^2\cdot \frac{(n+m)^{1/2+\delta}}{z^{1/2}})$, for any constant $\delta>0$ and trade-off parameter $z$. The details are deferred to the full version.
%Sec.~\ref{sec:small opt 2D halfplanes}.

\subsubsection*{Data structures.} To construct our main data structure, we recursively apply Matou\v{s}ek's Partition Theorem \cite{matouvsek1992efficient} as stated below, and decompose the problem into subproblems. The original version of Matou\v sek's theorem does not guarantee disjointness of cells, but a later version by
Chan~\cite{Chan12DCG} does.

%\Subhash{In the following theorem, do we need to say something about the "geometry" of these $b$ cells? Are they "triangles" for instance?}
\begin{theorem}[Matou\v{s}ek's Partition Theorem]\label{thm:partition short}
Given a set $S$ of $m$ points in $\R^2$, for any positive integer $b\le m$, we can partition $S$ into $b$ subsets $S_i$ each with size $O(\frac{m}{b})$ and find $b$ disjoint triangular cells $\Delta_i\supset S_i$, such that any halfplane crosses (i.e., the boundary intersects) $O(\sqrt{b})$ cells. The partition can be constructed in $O(m^{1+\delta})$ time.
\end{theorem}

%\TIMOTHY{do we need disjointness of cells? if so, need to cite my paper on optimal partition trees...}


Intuitively, with subproblems defined with this partition, any inserted/deleted halfplane $h$ only affects a small fraction of the subproblems. More precisely, we use Theorem~\ref{thm:partition short} to partition the set of points $S$ into $b$ cells $\Delta_i$, each containing a subset $S_i$ of $O(\frac{m}{b})$ points, where $b=N^{\delta_0}$ for sufficiently small constant $\delta_0$. Any halfplane will cross $O(\sqrt{b})$ cells, so each cell is crossed by $O(\frac{n\cdot \sqrt{b}}{b})=O(\frac{n}{\sqrt{b}})$ halfplanes in $\mathcal{H}$ on average. Call a cell \emph{good} if it crosses $\leq g\cdot \frac{n}{\sqrt{b}}$ halfplanes (for a sufficiently large constant $g$), otherwise \emph{bad}. Thus, there are only $O(\frac{n\sqrt{b}}{gn/\sqrt{b}})=O(\frac{b}{g})$ bad cells.
 
For the problem instance $(S,\mathcal{H})$, we construct the range searching data structures required by the small $\mathsf{opt}$ algorithm, and maintain an (implicit) $O(1)$-approximate solution $\mathcal{H}_{\mathrm{appx}}$. For each good cell $\Delta_i$, let $\mathcal{H}_i$ be the set of halfplanes crossing $\Delta_i$; we recursively solve the subproblem $(S_i,\mathcal{H}_i)$. We also recursively solve the subproblem $(S_{\mathrm{bad}},\mathcal{H})$ on the union of bad cells, where $S_{\mathrm{bad}}=\bigcup_{i:~\text{cell}~i~\text{bad}} S_i$. The total number of points decreases by a constant fraction, since $|S_{\mathrm{bad}}|=\sum_{i:~\text{cell}~i~\text{bad}}|S_i|\leq O(\frac{b}{g}\cdot \frac{m}{b})=O(\frac{m}{g})$.
%Although the number of halfplanes in the subproblem will not necessarily decrease, 

%The construction time is $T(m,n)=O(m^{1/3}n^{4/3}\cdot N^{O(\delta)})$.

\subsubsection*{Update.} When we insert/delete a halfplane $h$, we recurse in the $O(\sqrt{b})$ good cells $\Delta_i$ crossed by $h$, to recompute the approximate solutions $\mathcal{H}_{\mathrm{appx}}(S_i)$. We also recurse in the subproblem $(S_{\mathrm{bad}},\mathcal{H})$ for the union of bad cells, and recompute $\mathcal{H}_{\mathrm{appx}}(S_{\mathrm{bad}})$. We update the range searching data structure $\tilde{\mathcal{D}}^*$ required by the small $\mathsf{opt}$ algorithm, using $\widetilde{O}(z)$ time.

To reconstruct the approximate solution $\mathcal{H}_{\mathrm{appx}}$ we proceed as follows. If $\mathsf{opt}\leq O(b\log N)$, we use the small $\mathsf{opt}$ algorithm to recompute $\mathcal{H}_{\mathrm{appx}}$ from scratch. The condition $\mathsf{opt}\overset{?}{\leq }O(b\log N)$ can be tested by the small $\mathsf{opt}$ algorithm itself. Otherwise $\mathsf{opt}=\Omega(b\log N)$, and we can afford a larger additive error, so we return the union of the $O(1)$-approximate solutions for the good cells $S_i$ and the union of the bad cells $S_\mathrm{bad}$, i.e., let $\mathcal{H}_{\mathrm{appx}}=\bigcup_{i:~\text{cell}~i~\text{good}}\mathcal{H}_{\mathrm{appx}}(S_i)\cup \mathcal{H}_{\mathrm{appx}}(S_{\mathrm{bad}})$, which is stored implicitly.
(One special case is when there exists a halfplane $h$ that contains the cell $\Delta_i$, we include $h$ instead of $\mathcal{H}_{\mathrm{appx}}(S_i)$ in the solution $\mathcal{H}_{\mathrm{appx}}$.)

We rebuild the whole data structure every $\frac{gn}{\sqrt{b}}$ halfplane updates, so that good cells will not become bad. By setting $z=(n+m)^{1/3}$, the amortized cost per update is $\frac{T(m,n)}{gn/\sqrt{b}}+\tilde{O}(b^2\cdot \frac{(n+m)^{1/2+\delta}}{z^{1/2}})+\tilde{O}(z)=O(m^{1/3}n^{1/3}\cdot N^{O(\delta)})$, where $T(m,n)$ represents the construction time.

When we delete a point $p$, if $p$ is contained in a good cell $\Delta_i$, we recurse in the subproblem within $\Delta_i$ to recompute $\mathcal{H}_{\mathrm{appx}}(S_i)$. Otherwise $p$ is contained in a bad cell, so we recurse in the subproblem $(S_{\mathrm{bad}},\mathcal{H})$ and recompute $\mathcal{H}_{\mathrm{appx}}(S_{\mathrm{bad}})$. Then we recompute $\mathcal{H}_{\mathrm{appx}}$, using the procedure described above. We update the range searching data structure $\tilde{\mathcal{D}}$ required by the small $\mathsf{opt}$ algorithm, using $\widetilde{O}(z)$ time.

Let $U(m,n)$ denote the update time for $m$ points and $n$ halfplanes. It satisfies the recurrence
$$U\left(m,n\right)=O\left(\sqrt{b}\right)\cdot U\left(O\left(\frac{m}{b}\right),\frac{gn}{\sqrt{b}}\right)+U\left(O\left(\frac{m}{g}\right),n\right)+O\left(m^{1/3}n^{1/3}\cdot N^{O(\delta)}\right),$$
which solves to $U(m,n)=O(m^{1/3}n^{1/3}\cdot N^{O(\delta)})$ for $m\leq n$.
%. The running time is dominated by the costs at the lowest level, so for $m\leq n$

\subsubsection*{Approximation factor analysis.} The key observation here is that the boundary of the optimal solution $\mathcal{H}_{\mathrm{opt}}$ for $(S,\mathcal{H})$ must form a convex chain. As each cell is a triangle, it can only intersect the optimal convex chain $O(1)$ times, thus the $b$ disjoint cells will partition $\mathcal{H}_{\mathrm{opt}}$ into $O(b)$ pieces. If we take the union of the optimal solutions in all the cells, the additive error is at most $O(b)$.

If $\mathsf{opt}=\Omega(b\log N)$, we can afford the additive error. Otherwise we use the small $\mathsf{opt}$ algorithm to compute $\mathcal{H}_{\mathrm{appx}}$ from scratch. The multiplicative error grows by a factor at most $1+\frac{1}{\log N}$ at each level, and the recursion depth is $O(\log N)$, so the global multiplicative error is $O(1)$.

\begin{theorem}
There exists a data structure for $O(1)$-approximate dynamic 2D halfplane set cover that supports halfplane insertion/deletions and point deletions in amortized $O(n^{2/3+\delta})$ time w.h.p.\ for any constant $\delta>0$, and can answer size and reporting queries in $O(1)$ and $O(\mathsf{opt})$ time, respectively.
\end{theorem}

The issue with point insertions is we need to rebuild the whole structure every $O(\frac{m}{b})$ point insertions to bound the cell sizes, which is costly when $m$ is small. We resolve this issue using the \emph{logarithmic method}~\cite{bentley1980decomposable} but with a non-trivial base case, and finally obtain $O(n^{17/23+\delta})$ update time for all four types of updates.





\section{Weighted Interval Set Cover}
In this section, we present the first dynamic data structure with sub-linear update and constant factor approximation of weighted interval set cover.
Let $(S,\mathcal{I})$ be a dynamic weighted interval set cover instance where each interval $I \in \mathcal{I}$ has a weight $w(I) \geq 0$.
We show how to design a data structure $\mathcal{D}$ that maintains a $(3+\varepsilon)$-approximate solution for $(S,\mathcal{I})$.
Again, w.l.o.g., we assume that the points in $S$ are always in the point range $[0,1]$.
We say an interval in $\mathcal{I}$ is \textit{left} (resp., \textit{right}) \textit{one-sided} if it contains the left (resp., right) end of the point range $[0,1]$.

Let us first figure out the main difficulty of dynamic weighted interval set cover compared to the unweighted version.
As in the unweighted case, we partition the point range $[0,1]$ into portions $J_1,\dots,J_r$ such that each $J_i$ contains $O(n/r)$ points in $S$ and $O(n/r)$ endpoints of intervals in $\mathcal{I}$, and define $S_i = S \cap J_i$ and $\mathcal{I}_i = \{I \in \mathcal{I}: I \cap J_i \neq \emptyset \text{ and } J_i \nsubseteq I\}$.
Suppose we have sub-structures $\mathcal{D}_1,\dots,\mathcal{D}_r$ that can maintain ``good'' solutions for the sub-instances $(S_1,\mathcal{I}_1),\dots,(S_r,\mathcal{I}_r)$.
In the unweighted case, we construct a solution for $(S,\mathcal{I})$ in two ways: when $\mathsf{opt}$ is small, we use the output-sensitive algorithm of Lemma~\ref{lem-intos} to explicitly compute an optimal set cover; when $\mathsf{opt}$ is large, we construct a set cover by (essentially) taking the union of the solutions maintained in the sub-structures, which can be shown to have an $O(r)$ additive error (Fact~\ref{fact-intquality}).
Unfortunately, neither of the two ways applies to the weighted version.
First, we do not have an output-sensitive algorithm for weighted interval set cover analog to the one in Lemma~\ref{lem-intos}.
Second, we are not able to bound the additive error of the union of the solutions maintained in the sub-structures, mainly because the cost of a solution is now the total weight instead of the size.
Therefore, we need new ideas to construct the set cover of $(S,\mathcal{I})$, provided the solutions of the sub-instances.

Our basic idea is to obtain the solution for $(S,\mathcal{I})$ using a ``block-wise'' dynamic programming on $J_1,\dots,J_r$: we view each portion $J_i$ and the corresponding sub-instance $(S_i,\mathcal{I}_i)$ as a \textit{block} and try to cover these blocks optimally using the solutions of the sub-instances together with some ``long'' intervals in $\mathcal{I}$ each of which covers some portions in $\{J_1,\dots,J_r\}$.
Formally, let $\mathcal{I}_i^*$ be the solution of the sub-instance $(S_i,\mathcal{I}_i)$ maintained by $\mathcal{D}_i$.
We consider the solutions of $(S,\mathcal{I})$ of the form $\mathcal{I}_\text{long}^* \sqcup (\bigsqcup_{i \in P} \mathcal{I}_i^*)$ where $P \subseteq [r]$ and $\mathcal{I}_\text{long}^* \subseteq \mathcal{I}$ such that for any $i \in [r] \backslash P$ there exists an interval $I \in \mathcal{I}_\text{long}^*$ with $J_i \subseteq I$.
First, we observe that the optimal solution of this form can be found in $\widetilde{O}(r^{O(1)})$ time using DP\@.
To see this, for each $t \in [r]$, we define a sub-problem $\mathsf{Prob}_t$ as computing a minimum-cost set of the form $\mathcal{I}_\text{long}^* \sqcup (\bigsqcup_{i \in P} \mathcal{I}_i^*)$ such that $P \subseteq [t]$ and $\mathcal{I}_\text{long}^* \subseteq \mathcal{I}$ such that for any $i \in [t] \backslash P$ there exists an interval $I \in \mathcal{I}_\text{long}^*$ with $J_i \subseteq I$.
To solve the sub-problem $\mathsf{Prob}_t$, we consider the portion $J_t$.
We have two choices: \textbf{(i)} including $t$ in $P$ and including $\mathcal{I}_t^*$ to the solution, or \textbf{(ii)} including in $\mathcal{I}_\text{long}^*$ an interval $I \in \mathcal{I}$ that covers $J_t$.
If we choose \textbf{(i)}, then the remaining problem to be solved is exactly $\mathsf{Prob}_{t-1}$.
If we choose \textbf{(ii)}, then the remaining problem becomes $\mathsf{Prob}_{\pi(I)}$ where $\pi(I) \in [t-1]$ is the largest index that $J_{\pi(I)} \nsubseteq I$.
Note that for choice \textbf{(ii)}, we cannot afford to enumerate all $I \in \mathcal{I}$ that covers $J_t$.
To avoid this, the key observation is that if there are $I,I' \in \mathcal{I}$ covering $J_t$ such that $\pi(I) = \pi(I')$ and $w(I) \leq w(I')$, then we can ignore $I'$ and only try $I$.
Therefore, for each index $i \in [t-1]$, we only need to try the minimum-weight interval $I \in \mathcal{I}$ covering $J_t$ such that $\pi(I) = i$; such an interval can be found in $\widetilde{O}(1)$ time if we store $\mathcal{I}$ in a (dynamic) 2D range-min data structure.
It follows that we can solve the sub-problem $\mathsf{Prob}_t$ in $\widetilde{O}(r)$ time, given that $\mathsf{Prob}_1,\dots,\mathsf{Prob}_{t-1}$ are already solved.
Solving $\mathsf{Prob}_r$ gives what we want.

How good is the optimal solution of the form $\mathcal{I}_\text{long}^* \sqcup (\bigsqcup_{i \in P} \mathcal{I}_i^*)$?
For convenience, let us assume that $\mathcal{I}_i^*$ is an \textit{optimal} solution of $(S_i,\mathcal{I}_i)$ for all $i \in [r]$.
With this assumption, we can easily see that the optimal solution of this form is a $3$-approximate solution of $(S,\mathcal{I})$.
Indeed, in any solution $\mathcal{I}'$ of $(S,\mathcal{I})$, for each $i \in [r]$, either $J_i$ is covered by a single interval in $\mathcal{I}'$ or $\mathcal{I}' \cap \mathcal{I}_i$ is a set cover of $(S_i,\mathcal{I}_i)$.
In other words, any solution can be written as the form $\mathcal{I}_\text{long}^* \cup (\bigcup_{i \in P} \mathcal{I}_i')$ where each $\mathcal{I}_i'$ is a set cover of $(S_i,\mathcal{I}_i)$, and $P \subseteq [r]$, $\mathcal{I}_\text{long}^* \subseteq \mathcal{I}$ satisfy that for any $i \in [r] \backslash P$ there exists an interval $I \in \mathcal{I}_\text{long}^*$ with $J_i \subseteq I$.
Note that in the disjoint union $\mathcal{I}_\text{long}^* \sqcup (\bigsqcup_{i \in P} \mathcal{I}_i')$, each interval in $\mathcal{I}_\text{long}^* \cup (\bigcup_{i \in P} \mathcal{I}_i')$ has at most three copies because any interval in $\mathcal{I}$ is contained in at most two $\mathcal{I}_i$'s.
Therefore, $\mathsf{cost}(\mathcal{I}_\text{long}^* \sqcup (\bigsqcup_{i \in P} \mathcal{I}_i^*)) \leq \mathsf{cost}(\mathcal{I}_\text{long}^* \sqcup (\bigsqcup_{i \in P} \mathcal{I}_i')) \leq 3\cdot \mathsf{cost}(\mathcal{I}_\text{long}^* \cup (\bigcup_{i \in P} \mathcal{I}_i'))$,
which implies that the optimal solution of the form $\mathcal{I}_\text{long}^* \sqcup (\bigsqcup_{i \in P} \mathcal{I}_i^*)$ is a $3$-approximate solution of $(S,\mathcal{I})$.
However, this conclusion is obtained under the assumption that $\mathcal{I}_i^*$ is an optimal solution of $(S_i,\mathcal{I}_i)$ for all $i \in [r]$.
Clearly, we cannot afford to let the sub-structures maintain optimal solutions for the sub-instances.
If we recursively build the sub-structures, the approximation factor will increase in every level of the recursion.
The main reason why this happens is the following.
In a solution of the form $\mathcal{I}_\text{long}^* \sqcup (\bigsqcup_{i \in P} \mathcal{I}_i^*)$, each interval $I$ can belong to $\mathcal{I}_\text{long}^*$ and (at most) two $\mathcal{I}_i^*$'s.
If each of the two $\mathcal{I}_i^*$'s only contains one copy of $I$, then $I$ is counted three times.
However, now each $\mathcal{I}_i^*$ is the solution maintained by a recursively built sub-structure $\mathcal{D}_i$, so $I$ can be further duplicated in each $\mathcal{I}_i^*$.
To avoid this, we need to prevent an interval that is already duplicated in the current level from being duplicated in the lower levels of the recursion.
To this end, we observe that if an interval is counted more than once in $\mathcal{I}_\text{long}^* \sqcup (\bigsqcup_{i \in P} \mathcal{I}_i^*)$, then it either belongs to two $\mathcal{I}_i$'s or covers at least one portion $J_i$.
In both cases, it becomes \textit{one-sided} intervals in the (at most) two sub-instances containing it.
Therefore, if we can avoid duplicating the one-sided intervals, we are done.
%To avoid this, we first need to figure out why this can happen.
Observe that the left/right one-sided intervals are nested, so we need at most one left one-sided interval and one right one-sided interval in our solution.
A natural idea is to guess the left (resp., right) one-sided interval $L \in \mathcal{I}$ (resp., $R \in \mathcal{I}$) used in an optimal solution, and then construct a (good) set cover for the points in $S \backslash (L \cup R)$ using the above block-wise DP approach.
There are two difficulties to be overcome: \textbf{(i)} how to apply DP in this case and \textbf{(ii)} we cannot afford to enumerate all possible $L$ and $R$ as there can be $\Omega(n)$ one-sided intervals in $\mathcal{I}$.

We first consider difficulty \textbf{(i)}.
Suppose we already have the left (resp., right) one-sided interval $L \in \mathcal{I}$ (resp., $R \in \mathcal{I}$).
Assume the right (resp., left) endpoint of $L$ (resp., $R$) lies in $J_{i^-}$ (resp., $J_{i^+}$).
Then the points to be covered are those in $S_{i^-} \backslash L,S_{i^-+1},\dots,S_{i^+-1},S_{i^+} \backslash R$.
For the points in $S_{i^-+1},\dots,S_{i^+-1}$, we have the solutions maintained by the sub-structures $\mathcal{D}_{i^-+1},\dots,\mathcal{D}_{i^+-1}$.
The only thing different from before is that we need to handle the points in $S_{i^-} \backslash L$ and $S_{i^+} \backslash R$.
We have the solution for $(S_{i^-},\mathcal{I}_{i^-})$ (resp., $(S_{i^+},\mathcal{I}_{i^+})$) maintained in $\mathcal{D}_{i^-}$ (resp., $\mathcal{D}_{i^+}$).
Although it covers the points in $S_{i^-} \backslash L$ (resp., $S_{i^+} \backslash R$), it might be much more expensive than an optimal set cover for $(S_{i^-} \backslash L,\mathcal{I}_{i^-})$ (resp., $(S_{i^+} \backslash R,\mathcal{I}_{i^+})$).
However, we observe that we can obtain a ``good'' set cover for $(S_{i^-} \backslash L,\mathcal{I}_{i^-})$ (resp., $(S_{i^+} \backslash R,\mathcal{I}_{i^+})$) by (temporarily) inserting the interval $L$ (resp., $R$) with weight 0 to the sub-instance $(S_{i^-},\mathcal{I}_{i^-})$ (resp., $(S_{i^+},\mathcal{I}_{i^+})$) and update $\mathcal{D}_{i^-}$ (resp., $\mathcal{D}_{i^+}$); with the weight-0 interval, the points in $S_{i^-} \cap L$ (resp., $S_{i^-} \cap R$) can be covered for free and the solution maintained in $\mathcal{D}_{i^-}$ (resp., $\mathcal{D}_{i^+}$) is a good set cover for $(S_{i^-} \backslash L,\mathcal{I}_{i^-})$ (resp., $(S_{i^+} \backslash R,\mathcal{I}_{i^+})$).
With the good set covers for $(S_{i^-} \backslash L,\mathcal{I}_{i^-})$ and $(S_{i^+} \backslash R,\mathcal{I}_{i^+})$, we are able to apply the block-wise DP.

Next, we consider difficulty \textbf{(ii)}.
To avoid enumerating all one-sided intervals, our idea is to classify the left (resp., right) one-sided intervals in $\mathcal{I}$ into groups according to their weights such that the intervals in each group has similar weights, and in each group only consider the one with the maximum coverage.
%the key observation is the following: if we have a set of left (resp., right) one-sided intervals whose weights are similar, then we can simply keep the one that has the maximum coverage, i.e., with the rightmost right (resp., leftmost left) endpoint, and discard the others.
%Indeed, instead of using an interval we discard, we can always use the one we keep, which only increases the approximation ratio a little bit.
%Based on this observation, what we do is to classify the left (resp., right) one-sided intervals in $\mathcal{I}$ into groups according to their weights such that the intervals in each group has similar weights, and then pick from each group the interval with the maximum coverage.
Specifically, we maintain an estimation $\mathsf{opt}^\sim$ of the optimum satisfying $\mathsf{opt} \leq \mathsf{opt}^\sim \leq n^{O(1)} \mathsf{opt}$; such an estimation can be easily maintained in $\widetilde{O}(1)$ time using our dynamic unweighted interval set cover data structure in Section~\ref{sec-shortint}.
We then define $\delta_0 = 0$, $\delta_1 = \varepsilon \mathsf{opt}^\sim/n^c$ for a sufficiently large constant $c$, and $\delta_i = (1+\varepsilon) \cdot \delta_{i-1}$ for $i > 1$.
Let $m$ be the smallest integer such that $\delta_m \geq \mathsf{opt}^\sim$, so $m = \widetilde{O}(\frac{1}{\varepsilon} \log \frac{1}{\varepsilon})$.
For each $i \in [m]$, among all the left (resp., right) one-sided intervals in $\mathcal{I}$ whose weights are in the range $[\delta_{i-1},\delta_i]$, we pick the one $L_i$ (resp., $R_i$) with the maximum coverage, i.e., the one with the rightmost right (resp., leftmost left) endpoint.
Let $\mathcal{L} = \{L_1,\dots,L_m\}$ and $\mathcal{R} = \{R_1,\dots,R_m\}$.
We observe that the sets $\mathcal{L}$ and $\mathcal{R}$ can be computed in $\widetilde{O}(m) = \widetilde{O}(\frac{1}{\varepsilon} \log \frac{1}{\varepsilon})$ time using a (dynamic) 2D range-min/max data structure.
Instead of enumerating all one-sided intervals, we only enumerate the ones in $\mathcal{L}$ and $\mathcal{R}$.
If the optimal solution uses a left one-sided interval $L$ with $w(L) \in [\delta_{i-1},\delta_i]$ for $i > 1$, we can use the interval $L_i \in \mathcal{L}$ instead, and the resulting error can be charged to $w(L)$ because $w(L_i)/w(L) \leq \delta_i/\delta_{i-1} = 1+\varepsilon$.
The only exception is that the left one-sided interval $L$ used in the optimal solution has weight in $[\delta_0,\delta_1]$.
In this case, we can use $L_1 \in \mathcal{L}$ instead, but we cannot charge the resulting error to $w(L)$ as $w(L_1)/w(L)$ is unbounded (for $\delta_0 = 0$).
However, $w(L_1)$ is at most $\delta_1 \leq \varepsilon \mathsf{opt}/n^{\Omega(1)}$ and thus including $L_1$ in our solution only results in a small \textit{additive} error.
As in the unweighted case, we can handle such additive error by using a smaller approximation factor $\tilde{\varepsilon} = \alpha \varepsilon$ for the sub-structures $\mathcal{D}_1,\dots,\mathcal{D}_r$.
%Using the estimation $\mathsf{opt}^\sim$ of the optimum, we can actually classify the one-sided intervals in $\mathcal{I}$ into $\widetilde{O}(1/\varepsilon)$ groups where the intervals in each group have similar weights.
%In each group, we only keep the interval with the maximum coverage.
%In this way, we obtain a set of $\widetilde{O}(1/\varepsilon)$ \textit{candidate} one-sided intervals, and we only need to enumerate these candidate intervals, which can be done much more efficiently.

To summarize, our data structure $\mathcal{D}$ is designed as follows.
We define the portions $J_1,\dots,J_r$ and the sub-instances $(S_1,\mathcal{I}_1),\dots,(S_r,\mathcal{I}_r)$ in the same way as in Section~\ref{sec-shortint}.
For each $(S_i,\mathcal{I}_i)$, we recursively build a sub-structure $\mathcal{D}_i$ with the approximation factor $\tilde{\varepsilon} = \alpha \varepsilon$.
Also, we maintain the sets $\mathcal{L}$ and $\mathcal{R}$ described above (which are re-computed after each update).
Same as in Section~\ref{sec-shortint}, the data structure $\mathcal{D}$ will be reconstructed after $n/r$ operations.
To construct a solution for $(S,\mathcal{I})$, we enumerate all pairs $(L,R)$ where $L \in \mathcal{L}$ and $R \in \mathcal{R}$.
For each pair $(L,R)$, we use the block-wise DP described above to compute a set cover of $(S,\mathcal{I})$ which uses $L$ and $R$.
Among all the set cover we compute, we pick the one of the minimum cost as our solution $\mathcal{I}_\text{appx}$.
With a careful analysis based on the above reasoning, we can show $\mathsf{cost}(\mathcal{I}_\text{appx}) \leq (3+\varepsilon) \cdot \mathsf{opt}$.
Storing $\mathcal{I}_\text{appx}$ for answering queries is the same as in the unweighted case.

\subsubsection*{Analysis.}
We now analyze the update time of our data structure $\mathcal{D}$.
Besides recursively updating the sub-structures, each update of $\mathcal{D}$ takes $\widetilde{O}(m^2 r^{O(1)}) = \widetilde{O}((\frac{1}{\varepsilon} \log \frac{1}{\varepsilon})^2 \cdot r^{O(1)})$ amortized time.
The number of recursive updates we need is $O(m^2) = \widetilde{O}((\frac{1}{\varepsilon} \log \frac{1}{\varepsilon})^2)$, because when we do DP for each pair $(L,R)$, we need to temporarily insert the interval $L$ (resp., $R$) to a sub-instance (and delete it afterwards).
The depth of the recursion is $O(\log_r n)$.
Thus, if we set $\alpha = 1- 1/\log_r n$, the approximation factor in any level of the recursion is $\Theta(\varepsilon)$.
Therefore, the recurrence for the update time is
\begin{equation*}
    U(n) = \widetilde{O}\left(\left(\frac{1}{\varepsilon} \log \frac{1}{\varepsilon}\right)^2\right) \cdot U(O(n/r)) + \widetilde{O}\left(\left(\frac{1}{\varepsilon} \log \frac{1}{\varepsilon}\right)^2 \cdot r^{O(1)}\right),
\end{equation*}
which solves to $U(n) = (\log n \cdot \frac{1}{\varepsilon} \log \frac{1}{\varepsilon})^{O(\log_r n)} \cdot r^{O(1)}$.
Setting $r = 2^{\sqrt{\log n \log\log n} + \sqrt{\log n \log(1/\varepsilon)}}$, we have $U(n,\varepsilon) = 2^{O(\sqrt{\log n \log\log n} + \sqrt{\log n \log(1/\varepsilon)})}$.

\begin{restatable}{theorem}{weightedint}
There exists a dynamic data structure for $(3+\varepsilon)$-approximate weighted interval set cover with $2^{O(\sqrt{\log n \log\log n} + \sqrt{\log n \log(1/\varepsilon)})}$ amortized update time and $\widetilde{O}(n)$ construction time, which can answer size, membership, and reporting queries in $O(1)$, $O(\log n)$, and $O(k \log n)$ time, respectively, where $n$ is the size of the instance and $k$ is the size of the maintained solution.
\end{restatable}




\section{Weighted Unit-Square Set Cover}
In this section, we present the first sublinear result for dynamic weighted unit-square set cover, which gets $O(1)$-approximation. It suffices to consider dynamic weighted quadrant set cover, since the reduction \cite{agarwal2020dynamic} still works in the weighted case.

Let $(S,\mathcal{Q})$ be a dynamic weighted quadrant set cover instance where $S$ is the set of points in $\mathbb{R}^2$ and $\mathcal{Q}$ is the set of weighted quadrants, and let $n=|S|+|\mathcal{Q}|$ denote the instance size. We use $w(q)$ to denote the weight of a quadrant $q$, and $w(\mathcal{Q})$ for the weight of a set $\mathcal{Q}$. W.l.o.g., assume the points in $S$ lie in the point range $[0,1]^2$. For simplicity, we assume the weights are positive integers bounded by $U=\mathrm{poly}(n)$.

Our idea is based on our unweighted solution for quadrant set cover as explained in Section~\ref{unweighted unit-square}, which recursively solve for smaller sub-instances and properly combine them to obtain the global solution. In particular, we will again partition the space into $r\times r$ rectangular grid cells. However, our previous solution relies on an output-sensitive algorithm, but such algorithm is not known in the weighted case. Therefore, we will introduce some new ideas.


\subsubsection*{Data structures.} We construct a data structure $\mathcal{D}$ that supports a more powerful type of query:
\begin{quote}
Given a query rectangle $t$, compute an $O(1)$-approximate weighted set cover for the points in $S\cap t$, using the quadrants in $\mathcal{Q}$.
\end{quote}

For a quadrant $q\in \mathcal{Q}$ intersecting a rectangular range $\Gamma$, we say it is \emph{trivial} (resp., \emph{nontrivial}) with respect to $\Gamma$ if the vertex of $q$ is outside (resp., inside) $\Gamma$. Similar to the observation in the unweighted case, our idea is that it suffices to only keep a small subset of the trivial quadrants. In particular, among all trivial quadrants with weights $\in [1,2^{i})$, there are (at most) four maximal quadrants in $\Gamma$, which we denote as $\mathcal{M}_{\Gamma,i}$. We store $\mathcal{M}_{[0,1]^2,i}$ for $i=1,\dots,\log U$, and only keep the nontrivial quadrants with respect to $[0,1]^2$ in $\mathcal{Q}$. The intuition is suppose among all trivial quadrants in the optimal solution for $\Gamma$, the maximum weight is $w$, then for an $O(1)$-approximate solution we can just include $\mathcal{M}_{\Gamma,\lceil\log w\rceil}$, and then compute an $O(1)$-approximate solution in the complement region, using only the nontrivial quadrants.
%The union of the quadrants in $\mathcal{M}_{\Gamma,\lceil\log w\rceil}$ will contain the union of all trivial quadrants in $\mathcal{I}_{\mathrm{opt}}$.

To build the data structure $\mathcal{D}$, we partition the space into $r\times r$ grid cells using horizontal/vertical lines, such that each row/column has size $O(\frac{n}{r})$. We recursively create a sub-instance for each row (resp. column) $i$, that contains all points in the row and all quadrants that are nontrivial with respect to the row.
%Recursively construct the data structures for each of the $r$ rows and columns.
%Also store the sets of maximal quadrants in the rows and columns.
%where the size of a range $\Gamma$ is defined as the total number of points in $S$ and vertices of quadrants in $\mathcal{Q}$ inside $\Gamma$
%Let $\Box_{i,j}$ be the cell in the $i$-th row and $j$-th column.

For each of the $O(r^4)$ grid-aligned rectangles $\Box_{i,j,k,l}=\bigcup_{i'=i}^k\bigcup_{j'=j}^l\Box_{i',j'}$, we maintain an (implicit) $O(1)$-approximate set cover $\mathcal{Q}_{\mathrm{appx}}(\Box_{i,j,k,l})$ within it, so that its weight can be retrieved in $O(1)$ time. 


\subsubsection*{Dynamic programming.} In the following, we show that given the substructures for the columns, we can efficiently compute an $O(1)$-approximate solution for each grid-aligned rectangle $\Box_{i,j,k,l}$, using DP.

Any set cover solution can be decomposed into four subsets, based on the four directions of the quadrants. The boundary of the union of each subset forms an orthogonal staircase curve.
%(as shown in Figure~\ref{})
%which we denote as $U_{\mathrm{sol}}^{\mathrm{NW}},U_{\mathrm{sol}}^{\mathrm{SW}},U_{\mathrm{sol}}^{\mathrm{NE}},U_{\mathrm{sol}}^{\mathrm{SE}}$, respectively.

Let $\ell_0,\dots,\ell_r$ denote the $r+1$ vertical grid lines, and obtain line $\ell_i^-$ by slightly shifting $\ell_i$ to the left. We use $f[i_0][q_{_{\nwarrow}}][q_{_{\swarrow}}][q_{_{\nearrow}}][q_{_{\searrow}}]$ to denote the weight of an $O(1)$-approximate set cover $\mathcal{Q}_{\mathrm{appx}}$ that covers all points in $\Box_{i,j,k,l}$ and to the left of $\ell_{i_0}$, such that when we decompose $\mathcal{Q}_{\mathrm{appx}}$ into four orthogonal staircase curves, $\ell_{i_0}^-$ intersects them at $q_{_{\nwarrow}},q_{_{\swarrow}},q_{_{\nearrow}},q_{_{\searrow}}$, respectively.

We decompose each quadrant $q\in \mathcal{Q}$ into two parts: a \emph{long} part aligned with the leftmost/rightmost vertical grid line that intersects $q$, and a remaining \emph{short} part fully contained in a column (i.e.\ nontrivial in the column). For each vertical grid line $\ell_i$, among all long quadrants aligned with $\ell_i$, it suffices to keep the lowest (resp., highest) quadrant with direction north (resp., south) with weight $\in [2^k,2^{k+1})$, for each $k$. We keep $O(r\log U)$ long quadrants in total. The approximation factor will only multiply by a constant.

To compute $f[i_0][q_{_{\nwarrow}}'][q_{_{\swarrow}}'][q_{_{\nearrow}}'][q_{_{\searrow}}']$ (corresponding to the set cover solution $\mathcal{Q}_{\mathrm{appx}}'$) where the quadrants $q_{_{\nwarrow}}',q_{_{\swarrow}}',q_{_{\nearrow}}',q_{_{\searrow}}'$ are long, we guess that the four orthogonal staircase curves corresponding to $\mathcal{Q}_{\mathrm{appx}}'$ intersect $\ell_{i_0-1}^-$ at the four long quadrants $q_{_{\nwarrow}},q_{_{\swarrow}},q_{_{\nearrow}},q_{_{\searrow}}$. The set cover solution corresponding to $f[i_0-1][q_{_{\nwarrow}}][q_{_{\swarrow}}][q_{_{\nearrow}}][q_{_{\searrow}}]$ already covers all points to the left of $\ell_{i_0-1}$, so to obtain $\mathcal{Q}_{\mathrm{appx}}'$, we only need to cover the points between $\ell_{i_0-1}$ and $\ell_{i_0}$, using the short quadrants in column $i_0$. The region within $\Box_{i,j,k,l}$ and between $\ell_{i_0-1}$ and $\ell_{i_0}$ that are not covered by $q_{_{\nwarrow}}',q_{_{\swarrow}}',q_{_{\nearrow}}',q_{_{\searrow}}'$ is a rectangle $t'$.

In other words, $f[i_0][q_{_{\nwarrow}}'][q_{_{\swarrow}}'][q_{_{\nearrow}}'][q_{_{\searrow}}']$ can be computed by the formula
$$\min_{q_{_{\nwarrow}},q_{_{\swarrow}},q_{_{\nearrow}},q_{_{\searrow}}} \Big(f[i_0-1][q_{_{\nwarrow}}][q_{_{\swarrow}}][q_{_{\nearrow}}][q_{_{\searrow}}]+w(\mathcal{Q}_{\mathrm{appx}}(t'))+\sum_{d\in \{\nwarrow,\swarrow,\nearrow,\searrow\}} I[q_d'\neq q_d]\cdot w(q_d')\Big).$$
The weight of the approximate solution for $t'$ can be obtained by querying within column $i_0$.
%The final solution is the one with minimum weight among $f[r][q_{_{\nwarrow}}][q_{_{\swarrow}}][q_{_{\nearrow}}][q_{_{\searrow}}]$ for all possible long quadrants $q_{_{\nwarrow}},q_{_{\swarrow}},q_{_{\nearrow}},q_{_{\searrow}}$.

%We maintain pointers during the dynamic programming process about how the minimum weight is obtained, so that the actual solution can be easily recovered.

To compute the solution for $\Box_{i,j,k,l}$ we need to perform $(r\log U)^{O(1)}$ queries, since there are only $O(r\log U)$ choices for each of the long quadrants $q_{_{\nwarrow}}',q_{_{\swarrow}}',q_{_{\nearrow}}',q_{_{\searrow}}'$. The total running time for all $O(r^4)$ grid-aligned rectangles is $(r\log U)^{O(1)}\cdot Q(O(\frac{n}{r}))$.

As the recursion depth is constant, we can construct the whole data structure in $T(n)=\tilde{O}(n)$ time.
%\quad\newline

%Let $T(n)$ denote the construction time for the data structure $\mathcal{D}$ when the instance size is $n$. The construction time satisfies the recurrence
%$$T(n)=\sum_{i=1}^{2r} T(n_i)+\tilde{O}(n)+O(n^{O(\delta)}),$$
%where $n_i=O(\frac{n}{r})$ is the instance size of a row/column, and we have $\sum_{i=1}^{2r} n_i\leq 2n$. Set $r=N^{\delta}$ where $N$ is the global upper bound on the instance size and $\delta>0$ is an arbitrarily small constant. The recurrence solves to $T(n)=\tilde{O}(n)$.


\subsubsection*{Query.} Given a query rectangle $t$, we first \emph{guess} that the maximum weight among all trivial quadrants in the optimal solution is within $[2^{k-1},2^{k})$, and include $\mathcal{M}_{[0,1]^2,k}$ in our approximate solution. Let $t'$ denote the complement region of $\mathcal{M}_{[0,1]^2,k}$, it suffices to query for the rectangle $t_0=t\cap t'$, which can be decomposed into a grid-aligned rectangle $\Box_{i,j,k,l}$ and four rectangles $L_\leftarrow,L_\rightarrow,L_\uparrow,L_\downarrow$ each within a row/column, as shown in Figure~\ref{fig-annulus}. To compute the approximate solution for $t_0$, it suffices to take the union of the approximate solutions within $\Box_{i,j,k,l}$ and $L_\leftarrow,L_\rightarrow,L_\uparrow,L_\downarrow$. The approximation factor will grow only by a factor of~$5$.
%(for $O(\log U)$ choices of $k$)
%, i.e.\ let $\mathcal{Q}_{\mathrm{appx}}(t_0)=\mathcal{Q}_{\mathrm{appx}}(\Box_{i,j,k,l})\cup \mathcal{Q}_{\mathrm{appx}}(L_\leftarrow)\cup \mathcal{Q}_{\mathrm{appx}}(L_\rightarrow)\cup \mathcal{Q}_{\mathrm{appx}}(L_\uparrow)\cup \mathcal{Q}_{\mathrm{appx}}(L_\downarrow)$

$\mathcal{Q}_{\mathrm{appx}}(\Box_{i,j,k,l})$ has already been maintained. To compute $\mathcal{Q}_{\mathrm{appx}}(L_\uparrow)$ (and similarly for $L_\leftarrow,L_\rightarrow,L_\downarrow$), we perform a query on the rectangle $L_\uparrow$, using the substructure for the row $i-1$ containing $L_\uparrow$.

Let $Q(n)$ denote the query time for instance size $n$. It satisfies the recurrence
$$Q(n)=O(\log U)\cdot \left(4\cdot Q\left(O\left(\frac{n}{r}\right)\right)+O(1)\right).$$
The recursion depth is $O(\log_r n)=O(\frac{1}{\delta})$, so we have $Q(n)=O(\log U)^{O(\frac{1}{\delta})}=\log^{O(1)}n$. The approximation factor multiplies by a constant at each level, so the whole approximation factor is $O(1)^{O(\frac{1}{\delta})}=O(1)$.


\subsubsection*{Update.} When we insert/delete a quadrant $q$, recursively update the substructures for the row and column containing the vertex of $q$. Update the maximal quadrants $\mathcal{M}_{R_i,k}$ and $\mathcal{M}_{C_j,k}$ in the rows and columns, for $i,j\in [r]$ and $k=1,\dots,\log U$. Recompute the $O(1)$-approximate set cover solutions $\mathcal{Q}_{\mathrm{appx}}(\Box_{i,j,k,l})$ for each of the $O(r^4)$ grid-aligned rectangles $\Box_{i,j,k,l}$, using dynamic programming.
%in $(r\log U)^{O(1)}\cdot Q(O(\frac{n}{r}))$ time.


When we insert/delete a point $p$, recursively update the substructures for the row and column containing $p$, and recompute  $\mathcal{Q}_{\mathrm{appx}}(\Box_{i,j,k,l})$ for all grid-aligned rectangles $\Box_{i,j,k,l}$.

We reconstruct the entire data structure after every $\frac{n}{r}$ updates. The amortized cost is $\frac{T(n)}{n/r}=\tilde{O}(r)$.
%, so that the row and column sizes are always bounded by $O(\frac{n}{r})$.

Let $\mathcal{U}(n)$ denote the update time for instance size $n$. It satisfies the recurrence
$$\mathcal{U}(n)=2\mathcal{U}\left(O\left(\frac{n}{r}\right)\right)+(r\log U)^{O(1)}\cdot \mathcal{Q}\left(O\left(\frac{n}{r}\right)\right)+\tilde{O}(r),$$
which solves to $\mathcal{U}(n)=O(n^{O(\delta)})$.


\begin{theorem}
There exists a dynamic data structure for $O(1)$-approximate weighted unit-square set cover with $O(n^{\delta})$ amortized update time and $\tilde{O}(n)$ construction time, for any constant $\delta > 0$ (assuming polynomially bounded integer weights).
\end{theorem}


